Spherical symmetry in the kilonova AT2017gfo/GW170817

The mergers of neutron stars expel a heavy-element enriched fireball which can be observed as a kilonova. The kilonova's geometry is a key diagnostic of the merger and is dictated by the properties of ultra-dense matter and the energetics of the collapse to a black hole. Current hydrodynamical merger models typically show aspherical ejecta. Previously, Sr$^+$ was identified in the spectrum of the the only well-studied kilonova AT2017gfo, associated with the gravitational wave event GW170817. Here we combine the strong Sr$^+$ P Cygni absorption-emission spectral feature and the blackbody nature of kilonova spectrum, to determine that the kilonova is highly spherical at early epochs. Line shape analysis combined with the known inclination angle of the source also shows the same sphericity independently. We conclude that energy injection by radioactive decay is insufficient to make the ejecta spherical. A magnetar wind or jet from the black hole disk could inject enough energy to induce a more spherical distribution in the overall ejecta, however an additional process seems necessary to make the element distribution uniform

==> acknowledgements.tex <==
We thank Anja C. Andersen, Jonatan Selsing, Radek Wojtak, Katrine Frantzen,  Charles Steinhardt, and Christian Vogl for useful discussions. We thank the
ESO Director General for allocating Director’s Discretionary Time to this programme, and the ESO operation staff for support. 
D.W. is supported in part by Independent Research Fund Denmark grant DFF-7014-00017. The Cosmic Dawn Center is funded by the Danish National Research Foundation under grant number 140. A.B. and O.J. acknowledge support from the European Research Council (ERC) under the European Union’s Horizon 2020 research and innovation programme under grant agreement No.\ 759253. A.B. acknowledges support from Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) - Project-ID 279384907 - SFB 1245 and DFG - Project-ID 138713538 - SFB 881 (``The Milky Way System'', subproject A10) and support from the State of Hesse within the Cluster Project ELEMENTS. O.J. acknowledges computational support by the HOKUSAI computer center at RIKEN and by the VIRGO cluster at GSI. R.K. acknowledges support from the Academy of Finland (340613). S.A.S. acknowledges funding from the UKRI STFC Grant ST/T000198/1. D.P. acknowledges support from Israel Science Foundation (ISF) grant 541/17.


==> bibliography_sorted.tex <==
\begin{thebibliography}{10}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}

\bibitem{Eichler1989}
\bibinfo{author}{{Eichler}, D. et al.},
\newblock \bibinfo{title}{{Nucleosynthesis, neutrino
bursts and γ-rays from coalescing neutron stars}}.
\newblock \emph{\bibinfo{journal}{Nature}}
  \textbf{\bibinfo{volume}{340}}, \bibinfo{pages}{126-128}
  (\bibinfo{year}{1989}).
  
\bibitem{Barnes2013}
\bibinfo{author}{{Barnes}, J.}, \bibinfo{author}{{Mackie}, F.},
  \bibinfo{author}{{Kasen}, D.} \& \bibinfo{author}{{Schramm}, D.~N.}
\newblock \bibinfo{title}{{Effect of a High Opacity on the Light Curves of Radioactively Powered Transients from Compact Object Mergers.}}.
\newblock \emph{\bibinfo{journal}{Astrophys. J.}}
  \textbf{\bibinfo{volume}{775}}, \bibinfo{pages}{18}
  (\bibinfo{year}{2013}). 
 
\bibitem{Tanvir2013}
\bibinfo{author}{{Tanvir}, N. R. et al.},
\newblock \bibinfo{title}{{A ‘kilonova’ associated with the short-duration γ-ray burst GRB 130603B}}.
\newblock \emph{\bibinfo{journal}{Nature}}
  \textbf{\bibinfo{volume}{500}}, \bibinfo{pages}{547-549}
  (\bibinfo{year}{2013}).

\bibitem{Berger2013}
\bibinfo{author}{{Tanvir}, N.~R. et al.},
\newblock \bibinfo{title}{{n r-process Kilonova Associated with the Short-hard GRB 130603B}}.
\newblock \emph{\bibinfo{journal}{Astrophys. J. Lett.}}
  \textbf{\bibinfo{volume}{774}}, \bibinfo{pages}{L23}
  (\bibinfo{year}{2013}).    

\bibitem{Abbott2017b}
\bibinfo{author}{{Abbott}, B.~P. et al.}
\newblock \bibinfo{title}{{Gravitational Waves and Gamma-Rays from a Binary Neutron Star Merger: GW170817 and GRB 170817A}}.
\newblock \emph{\bibinfo{journal}{Astrophys. J. Lett.}}
  \textbf{\bibinfo{volume}{848}}, \bibinfo{pages}{L13}
  (\bibinfo{year}{2017}).

\bibitem{Pian2017}
\bibinfo{author}{{Pian}, E. et al.}
\newblock \bibinfo{title}{{pectroscopic identification of r-process nucleosynthesis in a double neutron-star merger.}}.
\newblock \emph{\bibinfo{journal}{Nature}}
  \textbf{\bibinfo{volume}{551}}, \bibinfo{pages}{67-70}
  (\bibinfo{year}{2017}).

\bibitem{Smartt2017}
\bibinfo{author}{{Smartt}, S.~J. et al.}
\newblock \bibinfo{title}{{A kilonova as the electromagnetic counterpart to a gravitational-wave source.}}.
\newblock \emph{\bibinfo{journal}{Nature}}
  \textbf{\bibinfo{volume}{551}}, \bibinfo{pages}{75-79}
  (\bibinfo{year}{2017}).

\bibitem{Coulter2017}
\bibinfo{author}{{Coulter}, D. A. et al.},
\newblock \bibinfo{title}{{The optical counterpart to a gravitational wave source}}.
\newblock \emph{\bibinfo{journal}{Science}}
  \textbf{\bibinfo{volume}{358}}, \bibinfo{pages}{1556–1558}
  (\bibinfo{year}{2017}).

\bibitem{Watson2019}
\bibinfo{author}{{Watson}, D. et al.},
\newblock \bibinfo{title}{{entification of strontium in the merger of two neutron stars}}.
\newblock \emph{\bibinfo{journal}{Nature}}
  \textbf{\bibinfo{volume}{574}}, \bibinfo{pages}{497–500}
  (\bibinfo{year}{2019}).

\bibitem{Abbott2017a}
\bibinfo{author}{{Abbott}, B.~P. et al.}, 
\newblock \bibinfo{title}{{A gravitational-wave standard siren measurement of the Hubble constant}}.
\newblock \emph{\bibinfo{journal}{Nature}} \textbf{\bibinfo{volume}{551}},
  \bibinfo{pages}{85--88} (\bibinfo{year}{2017}).
  


\end{thebibliography}

==> contributions.tex <==
A.S. and D.W. were the primary drivers of the project and wrote the main text
and developed the figures.  A.S. did all of the analysis and calculations,
wrote most of the Methods sections, and produced Figs.~1--4 and ED1--3.  OJ performed the hydrodynamical simulations and
produced \ref{fig:injection}.  O.J. and A.B. wrote the parts of the main text
and methods sections related to the simulations.  All authors were involved
in interpreting the results and discussed the results and commented on
and/or edited the text.



==> tables.tex <==
\begin{table*}[ht!]
\renewcommand{\arraystretch}{1.5} 
\centering
\begin{tabular*}{0.8\textwidth}{c @{\extracolsep{\fill}} ccccc}
\\ \hline \hline %& $T_{eff}$ & $v_{phot}$ &
Epoch    & $t-t_e$ [days] & $T_{eff}$ [K] & $v_{phot}$ [$c$] & $d_L$  [Mpc]  & $H_0 [\frac{km}{s Mpc}]$     \\ \hline 
1        & 1.43 & $5449 \pm 1$ & $0.2826 \pm 0.0003$ & $44.14_{-0.02}^{+0.11}$  & $65.5 \pm 3.0$  \\ \hline 
2        & 2.42 & $3961 \pm 2$ & $0.247 \pm 0.001$ & $44.14_{-0.17}^{+0.17}$  & $65.5 \pm 3.0$ \\ \hline 
Combined  & ------ & ------ & ------ & $-0.96 \pm 0.50$ & $65.5 \pm 3.0$   \\ 
\hline \hline
\end{tabular*}
    \caption{Time since merger, best fit inferred temperature $T_{eff}$, P-cygni velocity of photosphere $v_{phot}$, inferred luminosity distances and $H_0$ for first two epochs}
    \label{table:d_l}
\end{table*}


\begin{table}
\renewcommand{\arraystretch}{1.5} 
\centering
\begin{tabular*}{0.45\textwidth}{c @{\extracolsep{\fill}} ccccc}
\\ \hline \hline %& $T_{eff}$ & $v_{phot}$ &
Epoch    & $t-t_e$ [days] & $d_L$  [Mpc]  & $H_0 [\frac{km}{s Mpc}]$     \\ \hline 
1        & 1.43 & $44.20_{-0.02}^{+0.11}$  & $65.4 \pm 3.0$  \\ \hline 
2        & 2.42 & $44.14_{-0.17}^{+0.17}$  & $65.5 \pm 3.0$ \\ \hline 
1+2 & ------ & $44.14 \pm 0.50$ & $65.5 \pm 3.0$   \\ 
\hline \hline
\end{tabular*}
    \caption{Time since merger, inferred luminosity distances and $H_0$ for first two epochs of X-shooter spectra.}
    \label{table:d_l}
\end{table}




\begin{table}
\renewcommand{\arraystretch}{1.5} 
\centering
\begin{tabular*}{0.2\textwidth}{c @{\extracolsep{\fill}} c}
\\ \hline \hline %& $T_{eff}$ & $v_{phot}$ &
BNS mergers     & $\frac{\sigma_{H_0}}{H_0}$ \\ \hline 
1               &  $2.5 \%$  \\ \hline 
5               &  $1.1 \%$ \\ \hline 
10              &  $0.8 \%$ \\ 
\hline \hline
\end{tabular*}
    \caption{Future number of kilonova detected with GW and optical counterparts versus the expected fractional constraint attainable on $H_0$. All mergers are assumed to be uniformly distributed within the observable volume of the HLVK network during the O4-run, with identical intrinsic luminosity and peculiar velocity uncertainty as AT2017gfo.}
    \label{table:future}
\end{table}
